EFHQ: Multi-purpose ExtremePose-Face-HQ dataset

The existing facial datasets, while having plentiful images at near frontal views, lack images with extreme head poses, leading to the downgraded performance of deep learning models when dealing with profile or pitched faces. This work aims to address this gap by introducing a novel dataset named Extreme Pose Face High-Quality Dataset (EFHQ), which includes a maximum of 450k high-quality images of faces at extreme poses. To produce such a massive dataset, we utilize a novel and meticulous dataset processing pipeline to curate two publicly available datasets, VFHQ and CelebV-HQ, which contain many high-resolution face videos captured in various settings. Our dataset can complement existing datasets on various facial-related tasks, such as facial synthesis with 2D/3D-aware GAN, diffusion-based text-to-image face generation, and face reenactment. Specifically, training with EFHQ helps models generalize well across diverse poses, significantly improving performance in scenarios involving extreme views, confirmed by extensive experiments. Additionally, we utilize EFHQ to define a challenging cross-view face verification benchmark, in which the performance of SOTA face recognition models drops 5-37% compared to frontal-to-frontal scenarios, aiming to stimulate studies on face recognition under severe pose conditions in the wild.

==> tables/quant_reenactment.tex <==
\begin{table*}
\centering
\begin{tabular}{l|l|ccc|l|ccc} 
\hline
\multirow{2}{*}{}    & \multicolumn{4}{c|}{VoxCeleb1}  & \multicolumn{4}{c}{EFHQ (Ours)}         \\ 
\cline{2-9}
                     & Train Dataset  & $\mathcal{L}_1 \downarrow$ & AKD $\downarrow$ & AED $\downarrow$ & Train Dataset  & $\mathcal{L}_1 \downarrow$ & AKD $\downarrow$ & AED $\downarrow$  \\ 
\hline
\multirow{2}{*}{TPS} 
& VoxCeleb1      & \textbf{0.041} & \textbf{1.214} & \textbf{0.132} & VoxCeleb1 & 0.061 & 3.814 & 0.275    \\
& VoxCeleb1+EFHQ & \textbf{0.041} & 1.25 & 0.133 & VoxCeleb1+EFHQ & \textbf{0.051} & \textbf{1.963} & \textbf{0.214} \\ 
\hline
\multirow{2}{*}{LIA} 
& VoxCeleb1      & \textbf{0.044} & \textbf{1.342} & \textbf{0.138} & VoxCeleb1 & 0.059 & 3.807 & 0.266    \\
& VoxCeleb1+EFHQ & \textbf{0.044} & 1.398 & 0.142 & VoxCeleb1+EFHQ & \textbf{0.054} & \textbf{2.291} & \textbf{0.233} \\ 
\hline
\end{tabular}
    \vspace{-2mm}
\caption{Quantitative results of face reenactment models of two state-of-the-art methods (TPS and LIA) when training on VoxCeleb1 and the combined set VoxCeleb1+EFHQ. We present results evaluated either on VoxCeleb1 (left) or EFHQ (right) test sets.}
\label{tab:reenactment}
\end{table*}
